Summary of Discussion Sessions from "The Dusty Universe 2025: The Fifth Pandust Conference"

"The Dusty Universe: The Fifth Pandust Conference" took place in Tucson (AZ, USA) from November 10 until 14, 2025. The goal of this meeting was to get the dust community together to review where we are, hear exciting new results, and make plans for the future. The meeting encompassed all aspects of dust investigations including observations, theory, modeling, and laboratory studies. The conference consisted of invited review talks, contributed talks and posters. Science topics included interstellar dust (Milky Way & nearby galaxies), circumstellar dust (including Solar System & exoplanets), dust in Galaxies (including high-z), lifecycle of dust, and future needs (laboratory, theory, & observations), with a particular focus on results from JWST and ALMA, and on nanodust (including PAHs). On November 12th, we organized breakout discussion sessions covering a wide range of interesting dust-related topics. The purpose of this document is to capture the main topics/questions that were discussed, the key conclusions of these discussions, the challenges and possible solutions that were brought up, and the open questions that still remain to be answered. We hope that this document records our findings and challenges for the future generation.

==> AuxiliaryFiles/Referencing.tex <==
% !TEX root = ../BookTemplate.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{imakeidx}
\indexsetup{othercode=\small}
\makeindex[columns=2, intoc=false, columnseprule, title={}, options=-s ]

\RequirePackage[breaklinks, colorlinks=true, hypertexnames=true, linktoc=all]{hyperref}

\hypersetup{colorlinks,
		urlcolor={Url},
		citecolor={Cite},
		linkcolor={Link}}
